Offline Neural Contextual Bandits: Pessimism, Optimization and Generalization

Offline policy learning (OPL) leverages existing data collected a priori for policy optimization without any active exploration. Despite the prevalence and recent interest in this problem, its theoretical and algorithmic foundations in function approximation settings remain under-developed. In this paper, we consider this problem on the axes of distributional shift, optimization, and generalization in offline contextual bandits with neural networks. In particular, we propose a provably efficient offline contextual bandit with neural network function approximation that does not require any functional assumption on the reward. We show that our method provably generalizes over unseen contexts under a milder condition for distributional shift than the existing OPL works. Notably, unlike any other OPL method, our method learns from the offline data in an online manner using stochastic gradient descent, allowing us to leverage the benefits of online learning into an offline setting. Moreover, we show that our method is more computationally efficient and has a better dependence on the effective dimension of the neural network than an online counterpart. Finally, we demonstrate the empirical effectiveness of our method in a range of synthetic and real-world OPL problems.

==> body/main_proof.tex <==
\section{Proof of Main Result}
\label{section:main_proof}
In this section, we provide the proof of Theorem \ref{main_theorem}. The omitted proof is presented in the supplementary material. 

Let $\mathcal{D}_t = \{(\bm{x}_{\tau}, a_{\tau}, r_{\tau})\}_{1 \leq \tau \leq t}$, and let $\mathcal{F}_t = \sigma(\mathcal{D}_t)$ be the $\sigma$-algebra of $\mathcal{D}_t$ for all $ t \in [n]$. Note that $\hat{\pi}_t$ returned by Algorithm \ref{alg:neuralcb-sgd} is $\mathcal{F}_{t-1}$-measurable. Denote $\mathbb{E}_t[\cdot] = \mathbb{E}[\cdot | \mathcal{F}_t]$. Let the step sizes $\{\eta_t\}$ defined as in Theorem \ref{main_theorem} and the confidence trade-off parameters $\{\beta_t\}$ defined as in Algorithm \ref{alg:neuralcb-sgd}, we present main lemmas below which will culminate into the proof of the main theorem. 

\begin{lem}
There exists absolute constants $C_1, C_2 > 0$ such that for any $\delta \in (0,1)$, if $m$ satisfies 
\begin{align*}
    m \geq \max \bigg \{ \Theta(n \lambda^{-1} L^{11} \log^6 m), \Theta(L^6 n^4 K^4 \lambda_0^{-4} \log(KL(5n+1)/\delta) )\\
    \Theta( L^{-1} \lambda^{1/2} (\log^{3/2}( nKL^2 (5n + 1)/ \delta) \lor \log^{-3/2} m ))
     \bigg \},
\end{align*}
then with probability at least $1 - \delta$, it holds uniformly over all $t \in [n]$ that 
\begin{align*}
    &\subopt(\hat{\pi}_t; \bm{x}_t) \leq  2\beta_{t-1} \mathbb{E}_{a^*_t \sim \pi^*(\cdot|\bm{x}_t)} \left[ \| \nabla f_{\bm{W}^{(t-1)}}(\bm{x}_t \bm{e}_{a^*_t} ) \cdot m^{-1/2} \|_{ \bm{\Lambda}^{-1}_{t-1} }  | \mathcal{F}_t \right] \\ 
    &+ 2 C_1 t^{2/3} m^{-1/6} \log^{1/2} m L^{7/3} \lambda^{-1/2} + 2 \sqrt{2} C_2 \sqrt{nK} \lambda_0 ^{-1/2} m^{-11/6} \log^{1/2} m t^{1/6} L^{10/3} \lambda^{-1/6}.  
\end{align*}
\label{lemma:subopt_single_t_bound}
\end{lem}
Lemma \ref{lemma:subopt_single_t_bound} gives an upper bound on the sub-optimality of the returned step-dependent policy $\hat{\pi}_t$ on the observed context $\bm{x}_t$ for each $t \in [n]$. We remark that the upper bound depends on the rate at which the confidence width of the NTK feature vectors shrink along the direction of only the optimal actions, rather than any other actions. This is an advantage of pessimism where it does not require the offline data to be informative about any sub-optimal actions.  However, the upper bound depends on the unknown optimal policy $\pi^*$ while the offline data has been generated a priori by a different unknown behaviour policy. This distribution mismatch is handled in the next lemma. 
\begin{lem}
There exists an absolute constant $C_3 > 0 $ such that for any $\delta \in (0,1)$, if $m$ and $\lambda$ satisfy 
\begin{align*}
    \lambda \geq \max \{1, \Theta(L) \}, \hspace{0.5cm}  m \geq \max \bigg \{ \Theta( n \lambda^{-1} L^{11} \log^6 m), \Theta( L^6 n^4 K^4 \lambda_0^{-4} \log(nKL(5n+2)/\delta)) \\
    \Theta( L^{-1} \lambda^{1/2} (\log^{3/2}(nKL^2 (5n+2) / \delta) \lor \log^{-3/2} m ))
     \bigg \}, 
\end{align*}
then with probability at least $1 - \delta$, we have
\begin{align*}
    &\frac{1}{n} \sum_{t=1}^n \beta_{t-1} \mathbb{E}_{a^*_t \sim \pi^*(\cdot|\bm{x}_t)} \left[ \| \nabla f_{\bm{W}^{(t-1)}}(\bm{x}_t \bm{e}_{a^*_t} ) \cdot m^{-1/2} \|_{ \bm{\Lambda}^{-1}_{t-1} }  | \mathcal{F}_t \right] \\
    &\leq \frac{\sqrt{2} \beta_n \kappa}{\sqrt{n}} \sqrt{ \tilde{d} \log(1 + nK/\lambda)  + 1 + 2 C_2 C_3^2   n^{3/2} m^{-1/6} (\log m)^{1/2} L^{23/6} \lambda^{-1/6}} \\
    &+ \beta_n \kappa ( C_3 / \sqrt{2}) L^{1/2} \lambda_0^{-1/2} \log^{1/2}((5n + 2)/\delta),
\end{align*}
where $C_2$ is from Lemma \ref{lemma:subopt_single_t_bound}. 
\label{lemma:bound_sum}
\end{lem}
We also remark that the upper bound in Lemma \ref{lemma:bound_sum} scales linearly with $\sqrt{\tilde{d}}$ instead of with $\sqrt{p}$ if a standard analysis were applied. This avoids a vacuous bound as $p$ is large with respect to $n$.

The upper bounds in Lemma \ref{lemma:subopt_single_t_bound} and Lemma \ref{lemma:bound_sum} are established for the observed contexts only. The next lemma generalizes these bounds to the entire context distribution, thanks to the online-like nature of Algorithm \ref{alg:neuralcb-sgd} and an online-to-batch argument. In particular, a key technical property of Algorithm \ref{alg:neuralcb-sgd} that makes this generalization possible without a uniform convergence is that  $\hat{\pi}_t$ is $\mathcal{D}_{t-1}$-measurable and independent of $(\bm{x}_t, a_t, r_t)$. 

% \noindent There are some technical challenges to remark 
% \begin{itemize}
%     \item In offline learning, we need to handle generalization and distributional shift. Generalization is not a main problem in RL (@TODO: prove it), so it is highly non-trivial to obtain generalization in offline learning. 
%     \item We do not make any parametric assumption on the reward function rather than its boundedness 
%     \item To avoid strong parametric assumptions, we use overparameterized neural networks and thus $m$ is very large. Thus, we need to make sure that the generalization bound is not non-vacuous by making it independent of $m$
%     \item Here the feature mapping is adaptive to the training data, not static as in linear models or kernel functions, posing more challenging. 
% \end{itemize}


% Let $\mathcal{D}_t = \{(x_{\tau}, a_{\tau}, r_{\tau})\}_{1 \leq \tau \leq t}, \forall t \in [n]$. Let $\mathcal{D}_0 = \emptyset$ and $\hat{\pi}_0$ is a uniform policy. An online learner $\texttt{A}$ works as follows: At step $t \in [n]$, $\texttt{A}$ takes in $\mathcal{D}_{t-1}$ and $\hat{\pi}_{t-1}$ and produces a policy $\hat{\pi}_t$. 

\begin{lem}
For any $\delta \in (0,1)$, with probability at least $1-\delta$ over the randomness of $\mathcal{D}_n$, we have
% \begin{align*}
     $\mathbb{E} \left[ \subopt(\hat{\pi}) \right] \leq \frac{1}{n} \sum_{t=1}^n \subopt(\hat{\pi}_t, x_t) + \sqrt{ \frac{2}{n} \log(1/\delta) }. $
% \end{align*}
\label{lemma:online-to-batch}
\end{lem}
% \begin{rem}
% Note that we discard the last hypothesis $\theta_t$ for purely technical reasons. 
% \end{rem}
% \begin{proof}
% We follow \citep{DBLP:journals/tit/Cesa-BianchiCG04}. For each $t \in [n]$, define $\mathcal{F}_t = \sigma(\mathcal{D}_t)$, and 
% \begin{align*}
%     Z_t = \text{SubOpt}(\hat{\pi}_t) - \text{SubOpt}(\hat{\pi}_t, x_t).
% \end{align*}
% Since $\hat{\pi}_t$ is $\mathcal{F}_{t-1}$-measurable and is independent of $x_t$, and $x_t$ are i.i.d. samples (from $\rho$), we have $\mathbb{E} \left[  Z_t | \mathcal{F}_{t-1} \right] = 0, \forall t \in [n]$. Note that $-1 \leq Z_t \leq 1$. Then, the result directly follows from the Hoeffding-Azuma inequality. 
% \end{proof}
We are now ready to prove the main theorem. 
\begin{proof}[Proof of Theorem \ref{main_theorem}]
Combining Lemma \ref{lemma:subopt_single_t_bound}, Lemma \ref{lemma:bound_sum}, and Lemma \ref{lemma:online-to-batch} via the union bound, we have
\begin{align*}
    n \cdot \mathbb{E}[ \subopt(\hat{\pi}) ] &\leq  \kappa \sqrt{n}  \Gamma_1 \sqrt{\tilde{d} \log(1 + nK/\lambda)  + \Gamma_2} +  \kappa \sqrt{n} \Gamma_3 + \Gamma_4 + \Gamma_5 + \sqrt{2 n \log((10n+4)/\delta)}, \\ 
    &\leq  \kappa \sqrt{n}  \sqrt{\tilde{d} \log(1 + nK/\lambda)  + 2} +  \kappa \sqrt{n}  + 2 + \sqrt{2 n \log(10n+4)/\delta)}
\end{align*}
where $m$ is chosen to be sufficiently large as a polynomial of $(n,L, K, \lambda^{-1}, \lambda_0^{-1}, \log(1/\delta))$ such that 
\begin{align*}
    \Gamma_1 &:= 2 \sqrt{2} \sqrt{\lambda + C_3^2 n L} (n^{1/2} \lambda^{1/2} + (nK)^{1/2} \lambda_0^{-1/2}) \cdot m^{-1/2} \leq 1 \\
    \Gamma_2 &:= 1 + 2 C_2 C_3^2  n^{3/2} m^{-1/6} (\log m)^{1/2} L^{23/6} \lambda^{-1/6} \leq 2 \\ 
    \Gamma_3 &:= \Gamma_1 \sqrt{n} (C_3/\sqrt{2}) L^{1/2} \lambda_0^{-1/2} \log^{1/2}((10n + 4)/\delta) \leq 1 \\ 
    \Gamma_4 & := 2 C_1 n^{5/3} m^{-1/6} (\log m)^{1/2} L^{7/3} \lambda^{-1/2} \leq 1 \\ 
    \Gamma_5 &:= 2 \sqrt{2} C_2 (nK)^{1/2} \lambda_0^{-1/2} m^{-11/6} (\log m)^{1/2} n^{7/6} L^{10/3} \lambda^{-1/6} \leq 1.
\end{align*}
\end{proof}

% \begin{prop}[Generalization]
% With probability at least $1 - \delta$, we have 
% \begin{align*}
%     \text{SubOpt}(\hat{\pi }) \leq  \frac{1}{n} \sum_{t=1}^n \text{SubOpt}(\hat{\pi}_t; x_t) + 6 \sqrt{\frac{1}{n} \log \frac{2(n+1)}{\delta}}.
% \end{align*}
% \end{prop}
% \begin{proof}
% Follow \citep[Theorem~4]{DBLP:journals/tit/Cesa-BianchiCG04}.
% \end{proof}


% \noindent \textbf{Error decomposition}. 
% For each $t \in [n]$,  let $\bar{U}_t(x,a) = \langle g(x,a; \theta_{t-1}), \theta_{t-1} - \theta_0 \rangle + \beta_{t-1} \| g(x, a; \theta_{t-1})\|_{Z_{t-1}^{-1}}$, $\bar{L}_t(x,a) = \langle g(x,a; \theta_{t-1}), \theta_{t-1} - \theta_0 \rangle - \beta_{t-1} \| g(x, a; \theta_{t-1})\|_{Z_{t-1}^{-1}}$, $\mathcal{C}_t = \{\theta: \|\theta - \theta_0\|_{Z_t}  \leq \beta_t / \sqrt{m} \}$, denote $\hat{a}_t \sim \hat{\pi}_t(\cdot| x_t), a^*_t \sim \pi^*(\cdot|x_t)$, and $\mathbb{E}_t[\cdot] = \mathbb{E} [\cdot | \mathcal{F}_t]$, we have
% \begin{align*}
%     \text{SubOpt}(\hat{\pi}_t, x_t) &= \mathbb{E}_t h(x_t, a^*_t) - \mathbb{E}_t h(x_t, \hat{a}_t) \\
%     &= \mathbb{E}_t \langle  g(x_t,a_t^*; \theta_0), \theta^* - \theta_0 \rangle - \mathbb{E}_t \langle g(x_t,\hat{a}_t; \theta_0), \theta^* - \theta_0 \rangle \\ 
%     &\leq  \mathbb{E}_t  \langle g(x_t,a_t^*; \theta_{t-1}), \theta^* - \theta_0 \rangle - \mathbb{E}_t  \langle g(x_t,\hat{a}_t; \theta_{t-1}), \theta^* - \theta_0 \rangle \\
%     &+ \mathbb{E}_t  \| \theta^* - \theta_0 \|_2 \left( \| g(x_t,a_t^*; \theta_{t-1}) - g(x_t,a_t^*; \theta_0) \|_2 + \| g(x_t,\hat{a}_t; \theta_{t-1}) - g(x_t,\hat{a}_t; \theta_0) \|_2\right) \\
%     &\leq \mathbb{E}_t \langle g(x_t,a_t^*; \theta_{t-1}), \theta^* - \theta_0 \rangle - \mathbb{E}_t \langle g(x_t,\hat{a}_t; \theta_{t-1}), \theta^* - \theta_0 \rangle \\
%     &+ C_1 \| h \|_{H^{-1}}\cdot  m^{-1/6} \sqrt{\log m} t^{1/6} \lambda^{-1/6} L^{7/2}\\ 
%     &\leq \mathbb{E}_t \bar{U}_t(x_t, a^*_t) - \mathbb{E}_t \bar{L}_t(x_t, \hat{a}_t) + C_1 \| h \|_{H^{-1}} \cdot m^{-1/6} \sqrt{\log m} t^{1/6} \lambda^{-1/6} L^{7/2} \\ 
%     &\leq \mathbb{E}_t U_t(x_t, a^*_t) - \mathbb{E}_t L_t(x_t, \hat{a}_t) + C_1 \| h \|_{H^{-1}} \cdot m^{-1/6} \sqrt{\log m} t^{1/6} \lambda^{-1/6} L^{7/2} + O(m^{-1/6} n^{2/3}) \\ 
%     &=  \mathbb{E}_t U_t(x_t, a^*_t) - \mathbb{E}_t L_t(x_t, a_t^*) + (\mathbb{E}_t L_t(x_t, a_t^*) - \mathbb{E}_t L_t(x_t, \hat{a}_t)) \\
%     &+ C_1 \| h \|_{H^{-1}} \cdot m^{-1/6} \sqrt{\log m} t^{1/6} \lambda^{-1/6} L^{7/2} + 2 C_2 m^{-1/6} \sqrt{\log m} t^{2/3} \lambda^{-2/3} L^3 \\
%     &\leq 2 \beta_{t-1} \mathbb{E}_t  \| g(x_t, a^*_t; \theta_{t-1}) \|_{Z_{t-1}^{-1}} \\
%     &+ C_1 \| h \|_{H^{-1}} \cdot m^{-1/6} \sqrt{\log m} t^{1/6} \lambda^{-1/6} L^{7/2} + 2 C_2 m^{-1/6} \sqrt{\log m} t^{2/3} \lambda^{-2/3} L^3
% \end{align*}
% where 
% \begin{itemize}
%     \item the second equality holds due to that near initialization $h$ in the training data is almost linear in terms of its weight, 
%     \item the first inequality follows from a simple triangle inequality, \item the second inequality follows from that $\theta_*$ is close to $\theta_0$ and near initialization the gradient is close to that at initialization 
%     \item the third inequality follows $\theta^* \in \mathcal{C}_{t-1}$ and $\min_{x: \|x - b\|_A \leq c} \langle a, x \rangle = \langle a, b \rangle + c \|a\|_{A^{-1}}$
%     \item the fourth inequality follows from that $f$ in the training data is close to its first-order Taylor approximation and $\| \theta_{t-1} - \theta_0\|_2 \leq 2 \sqrt{t/(m \lambda)}$.
%     \item the last inequality follows from that $\hat{a}_t$ maximizes $L_t(x_t, a)$.
% \end{itemize}

% Now, we proceed with proving each individual claims above. We denote that $f \lesssim g $ if there is a absolute constant $C$ such that $f \leq C \cdot g$. The first result is that the reward function on the training data $\{(x_t, a_t)\}_{t=1}^n$ behaves as a linear function with the feature map $g(\cdot, \cdot; \theta_0)$ and weights $\theta_* - \theta_0$ where $\theta_*$ is near the initialization $\theta_0$. \\



